Fast Diffusion Model

Diffusion models (DMs) have been adopted across diverse fields with its remarkable abilities in capturing intricate data distributions. In this paper, we propose a Fast Diffusion Model (FDM) to significantly speed up DMs from a stochastic optimization perspective for both faster training and sampling. We first find that the diffusion process of DMs accords with the stochastic optimization process of stochastic gradient descent (SGD) on a stochastic time-variant problem. Then, inspired by momentum SGD that uses both gradient and an extra momentum to achieve faster and more stable convergence than SGD, we integrate momentum into the diffusion process of DMs. This comes with a unique challenge of deriving the noise perturbation kernel from the momentum-based diffusion process. To this end, we frame the process as a Damped Oscillation system whose critically damped state -- the kernel solution -- avoids oscillation and yields a faster convergence speed of the diffusion process. Empirical results show that our FDM can be applied to several popular DM frameworks, e.g., VP, VE, and EDM, and reduces their training cost by about 50% with comparable image synthesis performance on CIFAR-10, FFHQ, and AFHQv2 datasets. Moreover, FDM decreases their sampling steps by about 3x to achieve similar performance under the same samplers. The code is available at https://github.com/sail-sg/FDM.

==> tables/stepsize.tex <==
\begin{wraptable}{r}{0.5\textwidth}
\vspace{-1.2em}
\small
\centering
\caption{Ablation study on step size. VP $2 \times$ and VP $3 \times$ denote VP with double and triple step sizes, respectively.  
}
\begin{tabular}{lcccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{4}{c}{\textbf{Training Duration (Mimg)}} \\
\multicolumn{1}{c}{}                                 & 50      & 100   & 150    & 200    \\ \midrule
VP                                                   & 2.74    & 2.24                      & 2.19   & 2.15   \\
VP $2 \times$                                                & 3.12    & 2.49                      & 2.36   & 2.29   \\
VP $3 \times$                                                & 3.51    & 2.80                      & 2.54   & 2.42   \\
VP-FDM                                                  & 2.74    & 2.24                      & 2.13   & 2.08  \\
\bottomrule
\end{tabular}
\label{tab:stepsize}
% \vspace{-6pt}
\end{wraptable}

==> tables/warmup.tex <==
\begin{wraptable}{r}{0.5\textwidth}
\vspace{-1.2em}
\small
\caption{Effects of our loss weight warm-up strategy. 
Our loss weight improves the performance during the early stages of training.
}
\label{tab:warmup}
\centering
\begin{tabular}{lcccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{4}{c}{\textbf{Training Duration (Mimg)}} \\
\multicolumn{1}{c}{}                        & 50   & 100 & 150  & 200  \\ 
\midrule
EDM                                         & 5.76 & 1.99                    & 1.92 & 1.88 \\
EDM w/ $\hat{\lambda}(\sigma)$                      & 2.14 & 1.92                    & 1.89 & 1.87 \\ \midrule
FDM w/o $\hat{\lambda}(\sigma)$                     & 2.29 & 1.95                    & 1.85 & 1.82 \\
FDM                                         & 2.17 & 1.93                    & 1.83 & 1.79 \\
\bottomrule
\end{tabular}
% \vspace{-6pt}
\end{wraptable}
